Mapping Degeneration Meets Label Evolution: Learning Infrared Small Target Detection with Single Point Supervision

Training a convolutional neural network (CNN) to detect infrared small targets in a fully supervised manner has gained remarkable research interests in recent years, but is highly labor expensive since a large number of per-pixel annotations are required. To handle this problem, in this paper, we make the first attempt to achieve infrared small target detection with point-level supervision. Interestingly, during the training phase supervised by point labels, we discover that CNNs first learn to segment a cluster of pixels near the targets, and then gradually converge to predict groundtruth point labels. Motivated by this "mapping degeneration" phenomenon, we propose a label evolution framework named label evolution with single point supervision (LESPS) to progressively expand the point label by leveraging the intermediate predictions of CNNs. In this way, the network predictions can finally approximate the updated pseudo labels, and a pixel-level target mask can be obtained to train CNNs in an end-to-end manner. We conduct extensive experiments with insightful visualizations to validate the effectiveness of our method. Experimental results show that CNNs equipped with LESPS can well recover the target masks from corresponding point labels, {and can achieve over 70% and 95% of their fully supervised performance in terms of pixel-level intersection over union (IoU) and object-level probability of detection (Pd), respectively. Code is available at https://github.com/XinyiYing/LESPS.

==> new_13 <==
@inproceedings{WS1,
  title={Boxsup: Exploiting bounding boxes to supervise convolutional networks for semantic segmentation},
  author={Dai, Jifeng and He, Kaiming and Sun, Jian},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={1635--1643},
  year={2015}
}

@inproceedings{WS2,
  title={Multiscale combinatorial grouping},
  author={Arbel{\'a}ez, Pablo and Pont-Tuset, Jordi and Barron, Jonathan T and Marques, Ferran and Malik, Jitendra},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={328--335},
  year={2014}
}

@inproceedings{WS3,
  title={Weakly-and semi-supervised learning of a deep convolutional network for semantic image segmentation},
  author={Papandreou, George and Chen, Liang-Chieh and Murphy, Kevin P and Yuille, Alan L},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={1742--1750},
  year={2015}
}

@inproceedings{WS4,
  title={Simple does it: Weakly supervised instance and semantic segmentation},
  author={Khoreva, Anna and Benenson, Rodrigo and Hosang, Jan and Hein, Matthias and Schiele, Bernt},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={876--885},
  year={2017}
}

@article{WS5,
  title={Fully convolutional multi-class multiple instance learning},
  author={Pathak, Deepak and Shelhamer, Evan and Long, Jonathan and Darrell, Trevor},
  journal={arXiv preprint arXiv:1412.7144},
  year={2014}
}

@inproceedings{WS6,
  title={Constrained convolutional neural networks for weakly supervised segmentation},
  author={Pathak, Deepak and Krahenbuhl, Philipp and Darrell, Trevor},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={1796--1804},
  year={2015}
}

@inproceedings{WS7,
  title={From image-level to pixel-level labeling with convolutional networks},
  author={Pinheiro, Pedro O and Collobert, Ronan},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={1713--1721},
  year={2015}
}

